A Novel Decentralized Algorithm for Coordinating the Optimal Power and Traffic Flows with EVs based on Variable Inner Loop Selection

The electric power distribution network (PDN) and the transportation network (TN) are generally operated/coordinated by different entities. However, they are coupled with each other due to electric vehicle charging stations (EVCSs). This paper proposes to coordinate the operation of the two systems via a fully decentralized framework where the PDN and TN operators solve their own operation problems by sharing only limited information. Nevertheless, the operation problems generally are in mixed-integer programming (MIP) form. To the best of our knowledge, the most existing decentralized/distributed optimization algorithms, such as the alternating direction method of multipliers (ADMM), are not always guaranteed to converge for such MIP problems. Therefore, a novel fully decentralized optimization algorithm is proposed, whose contributions include: 1) it is applicable to MIP problems with convergence and optimality guaranteed for mild assumptions, 2) it only requires limited information exchange between PDN and TN operators, which will help preserve the privacy of the two systems and reduce the investment in building communication channels, and 3) it is fully decentralized so that all the computations are carried out by PDN operator and TN coordinator only. Simulations on the test cases show the efficiency and efficacy of the proposed framework and algorithm.

==> extra.tex <==
%As a result, the decentralized algorithm is required to have the capability to handle the integer-dependent boundary variables. Note that existing algorithms such as ADMM could not guarantee the optimality and convergence to MIP problems, let alone the integer-dependent boundary variable type MIP problems. Henceforth, in this paper, a mixed-integer boundary variable capable (MIBC) decentralized algorithm is proposed based on the SDM-GS-ALM algorithm \cite{boland2019parallelizable}. It is worth noting that the SDM-GS-ALM algorithm is not applicable to cases with integer-dependent boundary variables. The MIBC decentralized algorithm, utilized to coordinate the solutions of optimization models \eqref{CDEWN0P} and  \eqref{CDEWN0W}, is given in Algorithm 1. 
%\vspace{-3mm}
\begin{algorithm}[htbp]
\caption{MIBC Decentralized Algorithm}
\label{alg:euclid1}
%\begin{multicols}{2}
\begin{algorithmic}[1]
\\\textbf{Parameters initialization: }
\begin{enumerate}
    \item \textbf{Initial parameters: } Choose the initial parameters $ \epsilon, \rho, J, K$.\\
    \textbf{Starting point: }Choose $\boldsymbol{y}^0,\boldsymbol{\lambda _{p}}^0, \boldsymbol{\lambda _{w}}^0,\bm{\alpha}^0,\mathcal{D}_p:=\{\bm{x_{p}}^0\}, \mathcal{D}_w:=\{\bm{x_{w}}^0\},\check{\varphi}_p^0,\check{\varphi}_w^0$. Set $k=1$.
\end{enumerate}
\\\textbf{Iteration initialization: }Set $ \{\boldsymbol y, \boldsymbol{\lambda _{p}},\boldsymbol{\lambda _{w}}, \bm{\alpha}, \check {\varphi}_p, \check {\varphi}_w\}^k := \{\bm{y},\boldsymbol{\lambda _{p}},\boldsymbol{\lambda _{w}}, \bm{\alpha},\check {\varphi}_p, \check {\varphi}_w\}^{k-1}$.
\\\textbf{Continuous primal iteration: } Solve the following optimization problems \eqref{lr_lower1} and \eqref{lr_lower2} in parallel and then \eqref{yupdate} with the latest available updates of $\bm{p}^{\bm{\mathrm{l}}},\bm{p}^{\bm{\mathrm{p}}},\boldsymbol y,\boldsymbol{\lambda _{p}}, \boldsymbol{\lambda _{w}},\bm{\alpha}$. Repeat this step $J$ times.
\begin{subequations}
\begin{align}
 \bm{x_{p}}^k,\bm{p}^{\bm{\mathrm{l}}(k)}\gets \argmin_{\bm{x_{p}},\bm{p}^{\bm{\mathrm{l}}}} &\{ L_{\rho,p}\left( \bm{x_{p}}, \boldsymbol{y}^k,\boldsymbol{\lambda _{p}}^k \right): \nonumber \\
&\bm{x_{p}} \in \mathcal{D}_p\} \label{lr_lower1}\\
 \bm{x_{w}}^k,\bm{p}^{\bm{\mathrm{p}}(k)}\gets \argmin_{\bm{x_{w}},\bm{p}^{\bm{\mathrm{p}}}} &\{ L_{\rho,w}\left( \bm{x_{w}}, \boldsymbol{y}^k,\boldsymbol{\lambda _{w}}^k \right): \nonumber \\
& \bm{x_{w}} \in \mathcal{D}_w, \bm{\alpha} \in \bm{\alpha}^k\}  \label{lr_lower2}
\end{align}
\end{subequations}
\begin{equation}
\boldsymbol{y}^k \gets \min_{} \left\{  \left\|\bm{y}- \bm{p}^{\bm{\mathrm{l}}(k)}\right\|_2^2 + \left\| \bm{p}^{\bm{\mathrm{p}}(k)}-\bm{y} \right\|_2^2  \right\}     \label{yupdate}
\end{equation}
\\\textbf{MIP primal iteration: } Solve the following MIP subproblems \eqref{tilde1} and \eqref{tilde2}  in parallel
\begin{subequations}
\begin{align}
&\tilde{\varphi}_p \gets \check{\varphi}_p \left( \boldsymbol{\lambda _{p}}^k+\rho\left( \boldsymbol{y}^k-\bm{p}^{\bm{\mathrm{l}}(k)} \right) \right) \label{tilde1}, \\
&\tilde{\varphi}_w \gets \check{\varphi}_w \left( \boldsymbol{\lambda _{w}}^k+\rho\left(\bm{p}^{\bm{\mathrm{p}}(k)}-\boldsymbol{y}^k \right) \right). \label{tilde2}
\end{align}
\end{subequations}
And perform the following updates:
\begin{subequations}
\begin{align}
&\hat{ \bm{x}}_{\bm{p}} \gets \arg_{\bm{x_{p}}} \check{\varphi}_p \left( \boldsymbol{\lambda _{p}}^k+\rho\left( \boldsymbol{y}^k-\bm{p}^{\bm{\mathrm{l}}(k)} \right) \right), \nonumber \\
&\hat{ \bm{x}}_{\bm{w}}, \bm{\alpha}^k \gets \arg_{\bm{x_{w}}} \check{\varphi}_w \left( \boldsymbol{\lambda _{w}}^k+\rho\left(\bm{p}^{\bm{\mathrm{p}}(k)}-\boldsymbol{y}^k \right) \right), \nonumber \\
&\mathcal{D}_p \gets \left( \mathcal{D}_p \cup \{\hat{ \bm{x}}_{\bm{p}} \} \right), \nonumber \\
&\mathcal{D}_w \gets \left( \mathcal{D}_w \cup \{\hat{ \bm{x}}_{\bm{w}} \} \right), \nonumber \\
&\varepsilon_p^k \gets \hat{\varphi}_p \left( \boldsymbol{\lambda _{p}}^k, \bm{x_{p}}^k,\boldsymbol{y}^k \right)-\check{\varphi}_p^k, \nonumber \\
&\varepsilon_w^k \gets \hat{\varphi}_w \left( \boldsymbol{\lambda _{w}}^k, \bm{x_{w}}^k,\boldsymbol{y}^k \right)-\check{\varphi}_w^k. \nonumber 
\end{align}
\end{subequations}
\\\textbf{Stopping test: }If $\left( \varepsilon_p^k +\varepsilon_w^k \right)\le \epsilon$, Stop: $\left( \bm{x_{p}}^k, \bm{x_{w}}^k,\boldsymbol{y}^k,\boldsymbol{\lambda _{p}}^k,\boldsymbol{\lambda _{w}}^k,\bm{\alpha}^k,\check{\varphi}_p^k, \check{\varphi}_w^k \right)$ is the solution. Otherwise, continue.
\\\textbf{Iteration declaration: } The iteration is declared \textit{forward} iteration if the following inequality holds:
\begin{equation}
  (\hat{\varphi}_p+\hat{\varphi}_w) \ge (\tilde{\varphi}_p+\tilde{\varphi}_w) \ge (\check{\varphi}_p+\check{\varphi}_w). \label{declare_iteration}
\end{equation}
Perform the following updates if the iteration is declared \textit{forward}:
\begin{subequations}
\begin{align}
&\boldsymbol{\lambda _{p}}^k \gets \boldsymbol{\lambda _{p}}^k+\rho\left( \boldsymbol{y}^k-\boldsymbol{p}^{l(k)} \right) \nonumber \\
&\boldsymbol{\lambda _{w}}^k \gets \boldsymbol{\lambda _{w}}^k+\rho\left( \boldsymbol{p}^{p(k)} - \boldsymbol{y}^k \right) \nonumber \\
&\check{\varphi}_p^k \gets \tilde{\varphi}_p,~ \check{\varphi}_w^k \gets \tilde{\varphi}_w \nonumber
\end{align}
\end{subequations}
Otherwise, the iteration is declared \textit{neutral}: Algorithm continues without updates.
\algstore{myalg}
\end{algorithmic}
\end{algorithm}
\begin{algorithm}                     
\begin{algorithmic} [1]               
\algrestore{myalg}
\\\textbf{Auxiliary variable update: } If ${\alpha}_{n,t}^k-{\alpha}_{n,t}^{k-1} =1$, perform following update for all $n$ and $t$:
\begin{equation}
    {y}_{n,t}^k \gets {y}_{n,t}^a:a = \max \{\mathcal{M}\}, \mathcal{M} \subset \mathcal{K}_k. \nonumber
\end{equation}
If ${\alpha}_{n,t}^k-{\alpha}_{n,t}^{k-1} =0$, perform: ${y}_{n,t}^k \gets {y}_{n,t}^k$.
If ${\alpha}_{n,t}^k-{\alpha}_{n,t}^{k-1} =-1$, do: ${y}_{n,t}^k \gets 0$.
\\\textbf{Loop: }Set $k:=k+1$ and go back to Step 2.
\end{algorithmic}
%\end{multicols}
\end{algorithm}
\begin{comment}
\begin{table}[htbp]
\centering
\caption{Nomenclature: MIBC}
\label{nomenclature_MIBC}
%\resizebox{\linewidth}{!}{%
\begin{tabular}{lll}
\hline \hline
 & Symbol & Description \\ \hline
Indices & $\left( . \right)^k$ & Variables/parameters at iteration $k$. \\ \hline
\multirow{4}{*}{Sets} & ${D}_p$ & Subset of the convex hull of ${X_{p}}$. \\ \cline{2-3} 
 & ${D}_w$ & Subset of the convex hull of $\mathcal{X}_w$. \\ \cline{2-3} 
 & $M$ & Set of iteration $k$ with non-zero $\bm{y}$. \\ \cline{2-3}
 & $K_k$ & Set of iteration $k$, $\{1,2, \dots k\}$. \\ \hline
\multirow{4}{*}{Parameters}
 & $\epsilon$ & Convergence tolerance. \\ \cline{2-3} 
 & $K$ & Maximum number of main iterations. \\ \cline{2-3} 
 & $J$ & Maximum number of sub-iterations. \\ \cline{2-3} 
 & $\rho$ & Penalty parameter. \\ \hline
\multirow{4}{*}{Variables} & $\boldsymbol{\lambda}$ & Vector of Lagrangian multipliers. \\ \cline{2-3} 
 & $\bm{p^{\mathrm{p}}}$ & Vector of pump powers in a WDS. \\ \cline{2-3} 
 & $\bm{p^{\mathrm{l}}}$ & Vector of water pump load in a PDS. \\ \cline{2-3} 
 & $\bm{\alpha}$ & EdWFs on/off variable. \\ \hline \hline
\end{tabular}%
%}
\end{table}    
\end{comment}

%The algorithm is initialized by assigning convergence tolerance $\epsilon$ and penalty parameter $\rho$ in Step 1, along with maximum inner and outer loop iterations, $J$ and $K$, respectively. Note that Step 2 to Step 8 constitutes the outer loop while Step 3 is the inner loop. Moreover, the starting points for auxiliary variable ${\bm{y}}$, binary variable $\bm{\alpha}$, lagrangian multipliers $\boldsymbol{\lambda _{p}}^k$ and $\boldsymbol{\lambda _{w}}^k$, convex hulls subsets $\mathcal{D}_p$ and $\mathcal{D}_w$, and lagrangian lower bounds $\check {\varphi}_p$ and $\check {\varphi}_w$ are assigned. For the initial values of auxiliary variable ${\bm{y}}$ and lagrangian multipliers $\boldsymbol{\lambda _{p}}^k$ and $\boldsymbol{\lambda _{w}}^k$, we can use zero. For the initial values of OPF variables $\bm{x_{p}}$, OPS variables $\bm{x_{w}}$, and binary variables ${\bm{\alpha}}$, we can use any feasible solution. For the lagrangian lower bounds $\check {\varphi}_p$ and $\check {\varphi}_w$, we can use any small negative number.

%For the current iteration $k$, initial values of auxiliary variable ${\bm{y}}$, binary variable $\bm{\alpha}$, lagrangian multipliers $\boldsymbol{\lambda _{p}}^k$ and $\boldsymbol{\lambda _{w}}^k$, and lagrangian lower bounds $\check {\varphi}_p$ and $\check {\varphi}_w$ are set to that of the previous iteration $k-1$ in Step 2.

